Shared Experience Actor-Critic for Multi-Agent Reinforcement Learning

Exploration in multi-agent reinforcement learning is a challenging problem, especially in environments with sparse rewards. We propose a general method for efficient exploration by sharing experience amongst agents. Our proposed algorithm, called Shared Experience Actor-Critic (SEAC), applies experience sharing in an actor-critic framework. We evaluate SEAC in a collection of sparse-reward multi-agent environments and find that it consistently outperforms two baselines and two state-of-the-art algorithms by learning in fewer steps and converging to higher returns. In some harder environments, experience sharing makes the difference between learning to solve the task and not learning at all.

==> old_proof.tex <==
We provide the following derivation of SEAC policy loss, as shown in \Cref{eq:policyloss_shared}, for a fully observable two-agent Markov game
$$ \mathcal{M} = \left( \cN = \{1, 2\}, \cS, (A^1, A^2), \cP, (R^1, R^2)\right) $$
Similarly to \Cref{sec:background}, let $\cA = A^1 \times A^2$ be the joint action space and $A^1=A^2$.

\begin{assumption}[Symmetry Assumption: A1]\label{assumption:symmetry}
    We assume there exists a function $f: \cS \mapsto \cS$ such that
    \begin{equation*}
        \begin{split}
        &\forall s, s' \in \cS: \forall (a_1, a_2) \in \cA: R^1(f(s), (a_2, a_1), f(s')) = R^2(s, (a_1, a_2), s')\\
        \text{and }&\forall s, s' \in \cS: \forall (a_1, a_2) \in \cA: \cP(s, (a_1, a_2))(s') = \cP(f(s), (a_2, a_1))(f(s'))
        \end{split}
    \end{equation*}
    \end{assumption}
Intuitively, given a state $s$, $f(s)$ swaps the agents: agent $1$ is in place of agent $2$ and vice versa.

In the following, we use $\pi_1$ and $\pi_2$ to denote the policy of agent $1$ and agent $2$ which are conditioned on parameters $\phi_1$ and $\phi_2$, respectively. Similarly, we use $V^1$ and $V^2$ to denote the state value function of agents $1$ and $2$ which are conditioned on parameters $\theta_1$ and $\theta_2$.

\begin{assumption}[Reward Independence Assumption: A2]\label{assumption:independence}
    We assume that the rewards of an agent are only dependent on its own actions, and not the actions of others.\\ Therefore, for $(i, j) \in \{(1, 2), (2, 1)\}$:
        \begin{equation*}
            \E_{\substack{a_i \sim \pi_i\\a_j\sim\pi_j}}\left[R^i(s, (a_i, a_j), s')\right] \approx \E_{a_i \sim \pi_i}\left[R^i(s, (a_i, \cdot), \cdot)\right] \approx \E_{a_i,a_j\sim\pi_i}\left[R^i(s, (a_i, a_j), s')\right]
        \end{equation*}
\end{assumption}
Assumption~\ref{assumption:independence} above is not necessary, but has been used in SEAC for simplicity. At the end of the section, we discuss how the importance weights would be without this assumption.
\begin{lemma}[Importance Sampling]
\begin{equation*}
    \E_{x\sim p(x)}\left[ g(x) \right] = \int_x p(x)g(x) dx = \int_x q(x)\frac{p(x)}{q(x)} g(x) dx = \E_{x\sim q(x)}\left[  \frac{p(x)}{q(x)}g(x) \right]
\end{equation*}
\end{lemma}

During exploration, agent $1$ and $2$ follow policy $\pi_1$ and $\pi_2$ respectively. We will derive \Cref{eq:policyloss_shared,eq:valueloss_shared} for training $\pi_1$ using experience collected from agent $2$. The derivation for the other direction can be done by substituting agent indices.

Agent $2$ executes action $a_2$ in state $s$. Following Assumption~\ref{assumption:symmetry}, agent $1$ needs to reinforce $\pi_1(a_2, f(s))$. Notably, in state $f(s)$, $a_1$ is sampled by $\pi_2$. Importance sampling is used to correct for the behavioural policy. %The next state $s'$ is sampled from $\cP$, but is not written for brievety. 

\begin{derivation}[Actor Loss]

\begin{align*}
\begin{split}
    &\nabla_{\phi_1} J(\phi_1) = \E_{\substack{a_1 \sim\pi_2\\a_2 \sim \pi_1}} \left[ Q^1(f(s), a_2) \nabla_{\phi_1} \log \pi_1(a_2 | f(s))\right]\\
    &= \E_{a_1, a_2 \sim \pi_2} \left[ \frac{\pi_1(a_2 | f(s))}{\pi_2(a_2 | s))} Q^1(f(s), a_2) \nabla_{\phi_1} \log \pi_1(a_2 | f(s))\right]\\
    &= \E_{a_1, a_2 \sim \pi_2} \left[ \frac{\pi_1(a_2 | f(s))}{\pi_2(a_2 | s)} \left( R^1(f(s), (a_2, a_1), f(s')) + \gamma V^1(f(s')) \right) \nabla_{\phi_1} \log \pi_1(a_2 | f(s))\right]\\
    &\stackrel{A1}{=} \E_{a_1, a_2 \sim \pi_2} \left[ \frac{\pi_1(a_2 | f(s))}{\pi_2(a_2 | s)} \left( R^2(s, (a_1, a_2), s') + \gamma V^1(f(s')) \right) \nabla_{\phi_1} \log \pi_1(a_2 | f(s))\right]\\
    &\stackrel{A2}{\approx} \E_{\substack{a_1 \sim \pi_1\\ a_2 \sim \pi_2}} \left[ \frac{\pi_1(a_2 | f(s))}{\pi_2(a_2 | s)} \left( R^2(s, (a_1, a_2), s') + \gamma V^1(f(s')) \right) \nabla_{\phi_1} \log \pi_1(a_2 | f(s))\right]
\end{split}
\end{align*}

\end{derivation}

In the same manner, the value loss (note that the gradient does not flow through the target $V^1(f(s'))$).
\begin{derivation}[Value Loss]

\begin{align*}
\begin{split}
    % L(\theta_1) &= \E_{\substack{a_1\sim\pi_2\\a_2 \sim \pi_1}} \left[ ||V^1(f(s)) - y||^2 \right]\\
    % % &= \E_{a_1 \sim \pi_1} \left[ \sum_{a_2 \in A} \pi_2(a_2 | s) ||V^1(f(s)) - y||^2 \right]\\
    % % &= \E_{a_1 \sim \pi_1} \left[ \sum_{a_2 \in A} \frac{\pi_1(a_2 | f(s))}{\pi_1(a_2 | f(s))} \pi_2(a_2 | s) ||V^1(f(s)) - y||^2 \right]\\
    % &= \E_{a_1, a_2 \sim \pi_2} \left[\frac{\pi_1(a_2 | f(s))}{\pi_2(a_2 | s)} ||V^1(f(s)) - y||^2 \right]\\
    % &\stackrel{A2}{\approx} \E_{\substack{a_1\sim\pi_1\\ a_2 \sim \pi_2}} \left[\frac{\pi_1(a_2 | f(s))}{\pi_2(a_2 | s)} ||V^1(f(s)) - y||^2 \right]\\
    % %\text{where }y &= \E_{\substack{a_1 \sim \pi_1\\a_2 \sim \pi_2}}\left[R^1(f(s), (a_2, a_1), f(s')) + \gamma V^1(f(s')) \right]\\
    % %&= \E_{\substack{a_1 \sim \pi_1\\a_2 \sim \pi_2}}\left[R^2(s, (a_1, a_2), s') +\gamma V^1(f(s')) \right]
    % \text{where }y &= R^1(f(s), (a_2, a_1), f(s')) + \gamma V^1(f(s'))\\
    % % &= \E_{a_1 \sim \pi2}\left[R^2(s, (a_1, a_2), s') +\gamma V^1(f(s')) \right]\\
    % &\stackrel{A1}{=} R^2(s, (a_1, a_2), s') +\gamma V^1(f(s'))
    &L(\theta_1) = \E_{\substack{a_1\sim\pi_2\\a_2 \sim \pi_1}} \left[ ||V^1(f(s)) - \left( R^1(f(s), (a_2, a_1), f(s')) + \gamma V^1(f(s'))\right)||^2 \right]\\
    % &= \E_{a_1 \sim \pi_1} \left[ \sum_{a_2 \in A} \pi_2(a_2 | s) ||V^1(f(s)) - y||^2 \right]\\
    % &= \E_{a_1 \sim \pi_1} \left[ \sum_{a_2 \in A} \frac{\pi_1(a_2 | f(s))}{\pi_1(a_2 | f(s))} \pi_2(a_2 | s) ||V^1(f(s)) - y||^2 \right]\\
    &= \E_{a_1, a_2 \sim \pi_2} \left[\frac{\pi_1(a_2 | f(s))}{\pi_2(a_2 | s)} ||V^1(f(s)) - \left(R^1(f(s), (a_2, a_1), f(s')) + \gamma V^1(f(s'))\right)||^2 \right]\\
    &\stackrel{A2}{\approx} \E_{\substack{a_1\sim\pi_1\\ a_2 \sim \pi_2}} \left[\frac{\pi_1(a_2 | f(s))}{\pi_2(a_2 | s)} ||V^1(f(s)) - \left(R^1(f(s), (a_2, a_1), f(s')) + \gamma V^1(f(s'))\right)||^2 \right]\\
    %\text{where }y &= \E_{\substack{a_1 \sim \pi_1\\a_2 \sim \pi_2}}\left[R^1(f(s), (a_2, a_1), f(s')) + \gamma V^1(f(s')) \right]\\
    %&= \E_{\substack{a_1 \sim \pi_1\\a_2 \sim \pi_2}}\left[R^2(s, (a_1, a_2), s') +\gamma V^1(f(s')) \right]
    &\stackrel{A1}{=} \E_{\substack{a_1\sim\pi_1\\ a_2 \sim \pi_2}} \left[\frac{\pi_1(a_2 | f(s))}{\pi_2(a_2 | s)} ||V^1(f(s)) - \left(R^2(s, (a_1, a_2), s') + \gamma V^1(f(s'))\right)||^2 \right]
    %\text{where }y &= R^1(f(s), (a_2, a_1), f(s')) + \gamma V^1(f(s'))\\
    % &= \E_{a_1 \sim \pi2}\left[R^2(s, (a_1, a_2), s') +\gamma V^1(f(s')) \right]\\
    %&\stackrel{A1}{=} R^2(s, (a_1, a_2), s') +\gamma V^1(f(s'))
\end{split}
\end{align*}

\end{derivation}

The independence assumption, has been used to ignore that action $a_1$ should be sampled from $\pi_2$. Essentially, without correcting for this, agents are learning to play against themselves. The importance weights without this assumption would be \[ \frac{\pi_1(a_2 | f(s))\pi_2(a_1 |f(s))}{\pi_2(a_2 | s)\pi_1(a_1|s)} \] that are also correcting for the action selection policy of $a_1$.

==> proof.tex <==
We provide the following derivation of SEAC policy loss, as shown in \Cref{eq:policyloss_shared}, for a fully observable two-agent Markov game
$$ \mathcal{M} = \left( \cN = \{1, 2\}, \cS, (A^1, A^2), \cP, (R^1, R^2)\right) $$
As per \Cref{sec:background}, let $\bA = A^1 \times A^2$ be the joint action space and $A=A^1=A^2$.

In the following, we use $\pi_1$ and $\pi_2$ to denote the policy of agent $1$ and agent $2$ which are conditioned on parameters $\phi_1$ and $\phi_2$, respectively. We use $V^1$ and $V^2$ to denote the state value function of agents $1$ and $2$ which are conditioned on parameters $\theta_1$ and $\theta_2$.

%We can define transition probability functions $\cP^1$ and $\cP^2$ only defined over the individual actions of agents
%\begin{equation*}
%    \begin{split}
%        \cP^1(s, a_1, s') &=  \sum_{a_2 \in A^2} \left[\pi_2(a_2|s) \cP(s,(a_1,a_2), s')\right]\\
%        \cP^2(s, a_2, s') &=  \sum_{a_1 \in A^1} \left[\pi_1(a_1|s) \cP(s,(a_1,a_2), s')\right]
%    \end{split}
%\end{equation*}

%We can define reward functions $\bar{R}^1$ and $\bar{R}^2$ only defined over the individual actions of agents
%\begin{equation*}
%    \begin{split}
%        \bar{R}^1(s, a_1, s') &=  \sum_{a_2 \in A^2} \left[\pi_2(a_2|s) R^1(s,(a_1,a_2), s')\right]\\
%        \bar{R}^2(s, a_2, s') &=  \sum_{a_1 \in A^1} \left[\pi_1(a_1|s) R^2(s,(a_1,a_2), s')\right]
%    \end{split}
%\end{equation*}

%\begin{assumption}[Transition Independence Assumption: A1]
%\label{assumption:transition_independence}
%    We assume that agents perceive the environment dynamics defined by $\cP^1$ and $\cP^2$ ignoring the other agent's action selection.
%    \begin{equation*}
%        \begin{split}
%            \cP^1(s, a_1, s') &\approx  \cP(s,(a_1,\cdot), s')\\
%            \cP^2(s, a_2, s') &\approx  \cP(s,(\cdot,a_2), s')
%        \end{split}
%    \end{equation*}
%\end{assumption}
In order to account for different action distributions under policies $\pi_1$ and $\pi_2$, we use importance sampling (IS) defined for any function $g$ over actions
%\begin{lemma}[Importance Sampling: L1]
\begin{equation*}
    \E_{a\sim \pi_1(a|s)}\left[ g(a) \right] = \E_{a\sim \pi_2(a|s')}\left[\frac{\pi_1(a|s)}{\pi_2(a|s')} g(a) \right]
\end{equation*}
%\end{lemma}

which can be derived as follows
%\begin{proof}
\begin{equation*}
    \E_{a\sim \pi_1(a|s)}\left[ g(a) \right] = \int_a \pi_1(a|s) g(a) da = \int_a \frac{\pi_2(a|s')}{\pi_2(a|s')} \pi_1(a|s) g(a) da = \E_{a\sim \pi_2(a|s')}\left[  \frac{\pi_1(a|s)}{\pi_2(a|s')} g(a) \right]
\end{equation*}
%\end{proof}

\begin{assumption}[Reward Independence Assumption: A1]
\label{assumption:reward_independence}
    We assume that an agent perceives the rewards as dependent only on its own action. Other agents are perceived as part of the environment.
    \begin{equation*}
        \begin{split}
            \forall s, s' \in \cS: \forall a \in A: \hat{R}^1(s, a, s') &=  R^1(s,(a,\cdot), s')\\
            \forall s, s' \in \cS: \forall a \in A: \hat{R}^2(s, a, s') &=  R^2(s,(\cdot,a), s')
        \end{split}
    \end{equation*}
\end{assumption}

\begin{assumption}[Symmetry Assumption: A2]\label{assumption:symmetry}
    We assume there exists a function $f: \cS \mapsto \cS$ such that
    \begin{equation*}
        \begin{split}
        &\forall s, s' \in \cS: \forall (a_1, a_2) \in \bA: R^1(f(s), (a_2, a_1), f(s')) = R^2(s, (a_1, a_2), s')\\
        \text{and }&\forall s, s' \in \cS: \forall (a_1, a_2) \in \bA: \cP(s, (a_1, a_2))(s') = \cP(f(s), (a_2, a_1))(f(s'))
        \end{split}
    \end{equation*}
\end{assumption}
Intuitively, given a state $s$, $f(s)$ swaps the agents: agent $1$ is in place of agent $2$ and vice versa.

\begin{lemma}[Reward Symmetry: L1]\label{lemma:reward_symmetry}
    From these two assumptions, it follows that for any states $s, s' \in \cS$, and any action $a \in A$ the following holds:
    \begin{equation*}
        \begin{split}
            \hat{R}^1(f(s), a, f(s')) = \hat{R}^2(s, a, s')\\
            \hat{R}^2(f(s), a, f(s')) = \hat{R}^1(s, a, s')
        \end{split}
    \end{equation*}
\end{lemma}

\begin{proof}
    \begin{equation*}
        \begin{split}
            \hat{R}^1(f(s), a, f(s')) \stackrel{A1}{=} R^1(f(s), (a, \cdot), f(s')) \stackrel{A2}{=} R^2(s, (\cdot, a), s') \stackrel{A1}{=} \hat{R}^2(s, a, s')\\
            \hat{R}^2(f(s), a, f(s')) \stackrel{A1}{=} R^2(f(s), (\cdot, a), f(s')) \stackrel{A2}{=} R^1(s, (a, \cdot), s') \stackrel{A1}{=} \hat{R}^1(s, a, s')
        \end{split}
    \end{equation*}
\end{proof}

During exploration, agent $1$ and $2$ follow policy $\pi_1$ and $\pi_2$ respectively. We will derive \Cref{eq:policyloss_shared,eq:valueloss_shared} for training $\pi_1$ and $V^1$ using experience collected from agent $2$. The derivation for optimisation of $\pi_2$ and $V^2$ using experience of agent $1$ can be done analogously by substituting agent indices. Note that we only derive the off-policy terms of the SEAC policy and value loss. The on-policy terms of given losses are identical to A2C~\cite{Mnih2016AsynchronousLearning}.

Agent $2$ executes action $a_2$ in state $s$. Following Assumption~\ref{assumption:symmetry}, agent $1$ needs to reinforce $\pi_1(a_2, f(s))$. Notably, in state $f(s)$, $a_1$ is sampled by $\pi_2$, so importance sampling is used to correct for this behavioural policy. %The next state $s'$ is sampled from $\cP$, but is not written for brievety. 

\begin{proposition}[Actor Loss Gradient]
    \begin{equation*}
        \nabla_{\phi_1} \mathcal{L}(\phi_1) = \E_{a_2 \sim \pi_2} \left[ \frac{\pi_1(a_2 | f(s))}{\pi_2(a_2 | s)} \left( R^2(s, (\cdot, a_2), s') + \gamma V^1(f(s')) \right) \nabla_{\phi_1} \log \pi_1(a_2 | f(s))\right]
    \end{equation*}
\end{proposition}
\begin{proof}
    \begin{align*}
        \begin{split}
            &\nabla_{\phi_1} \mathcal{L}(\phi_1) = \E_{\substack{a_1 \sim\pi_2\\a_2 \sim \pi_1}} \left[ Q^1(f(s), a_2) \nabla_{\phi_1} \log \pi_1(a_2 | f(s))\right]\\
            &\stackrel{IS}{=} \E_{a_1, a_2 \sim \pi_2} \left[ \frac{\pi_1(a_2 | f(s))}{\pi_2(a_2 | s))} Q^1(f(s), a_2) \nabla_{\phi_1} \log \pi_1(a_2 | f(s))\right]\\
            &= \E_{a_1, a_2 \sim \pi_2} \left[ \frac{\pi_1(a_2 | f(s))}{\pi_2(a_2 | s)} \left( R^1(f(s), (a_2, a_1), f(s')) + \gamma V^1(f(s')) \right) \nabla_{\phi_1} \log \pi_1(a_2 | f(s))\right]\\
            &\stackrel{A1}{=} \E_{a_2 \sim \pi_2} \left[ \frac{\pi_1(a_2 | f(s))}{\pi_2(a_2 | s)} \left( \hat{R}^1(f(s), a_2, f(s')) + \gamma V^1(f(s')) \right) \nabla_{\phi_1} \log \pi_1(a_2 | f(s))\right]\\
            &\stackrel{L1}{=} \E_{a_2 \sim \pi_2} \left[ \frac{\pi_1(a_2 | f(s))}{\pi_2(a_2 | s)} \left( \hat{R}^2(s, a_2, s') + \gamma V^1(f(s')) \right) \nabla_{\phi_1} \log \pi_1(a_2 | f(s))\right]\\
            &\stackrel{A1}{=} \E_{a_2 \sim \pi_2} \left[ \frac{\pi_1(a_2 | f(s))}{\pi_2(a_2 | s)} \left( R^2(s, (\cdot, a_2), s') + \gamma V^1(f(s')) \right) \nabla_{\phi_1} \log \pi_1(a_2 | f(s))\right]
        \end{split}
    \end{align*}
\end{proof}

It should be noted that no gradient is back-propagated through the target $V^1(f(s'))$). In the same manner, the value loss, as shown in \Cref{eq:valueloss_shared}, can be derived as follows.

\begin{proposition}[Value Loss]
    \begin{equation*}
            \mathcal{L}(\theta_1) = \E_{a_2 \sim \pi_2} \left[\frac{\pi_1(a_2 | f(s))}{\pi_2(a_2 | s)} ||V^1(f(s)) - \left(R^2(s, (\cdot, a_2), s') + \gamma V^1(f(s'))\right)||^2 \right]
    \end{equation*}
\end{proposition}
\begin{proof}
    \begin{align*}
        \begin{split}
            &\mathcal{L}(\theta_1) = \E_{\substack{a_1\sim\pi_2\\a_2 \sim \pi_1}} \left[ ||V^1(f(s)) - \left( R^1(f(s), (a_2, a_1), f(s')) + \gamma V^1(f(s'))\right)||^2 \right]\\
            &\stackrel{IS}{=} \E_{a_1, a_2 \sim \pi_2} \left[\frac{\pi_1(a_2 | f(s))}{\pi_2(a_2 | s)} ||V^1(f(s)) - \left(R^1(f(s), (a_2, a_1), f(s')) + \gamma V^1(f(s'))\right)||^2 \right]\\
            &\stackrel{A1}{=} \E_{a_2 \sim \pi_2} \left[\frac{\pi_1(a_2 | f(s))}{\pi_2(a_2 | s)} ||V^1(f(s)) - \left(\hat{R}^1(f(s), a_2, f(s')) + \gamma V^1(f(s'))\right)||^2 \right]\\
            &\stackrel{L1}{=} \E_{a_2 \sim \pi_2} \left[\frac{\pi_1(a_2 | f(s))}{\pi_2(a_2 | s)} ||V^1(f(s)) - \left(\hat{R}^2(s, a_2, s') + \gamma V^1(f(s'))\right)||^2 \right]\\
            &\stackrel{A1}{=} \E_{a_2 \sim \pi_2} \left[\frac{\pi_1(a_2 | f(s))}{\pi_2(a_2 | s)} ||V^1(f(s)) - \left(R^2(s, (\cdot, a_2), s') + \gamma V^1(f(s'))\right)||^2 \right]
        \end{split}
    \end{align*}
\end{proof}
